Improving Face Recognition by Clustering Unlabeled Faces in the Wild

While deep face recognition has benefited significantly from large-scale labeled data, current research is focused on leveraging unlabeled data to further boost performance, reducing the cost of human annotation. Prior work has mostly been in controlled settings, where the labeled and unlabeled data sets have no overlapping identities by construction. This is not realistic in large-scale face recognition, where one must contend with such overlaps, the frequency of which increases with the volume of data. Ignoring identity overlap leads to significant labeling noise, as data from the same identity is split into multiple clusters. To address this, we propose a novel identity separation method based on extreme value theory. It is formulated as an out-of-distribution detection algorithm, and greatly reduces the problems caused by overlapping-identity label noise. Considering cluster assignments as pseudo-labels, we must also overcome the labeling noise from clustering errors. We propose a modulation of the cosine loss, where the modulation weights correspond to an estimate of clustering uncertainty. Extensive experiments on both controlled and real settings demonstrate our method's consistent improvements over supervised baselines, e.g., 11.6% improvement on IJB-A verification.

==> intro.tex <==
\textcolor{red}{[ELM: Alternative intro.] Semi-supervised learning attempts to improve performance by using massive unlabeled data sets to augment labeled data sets. In face recognition, a common assumption of semi-supervised methods is that there is no identity overlap between the unlabeled data and the labeled data. This seemingly mild assumption, however, violates the basic premise of semi-supervised learning--that nothing is known about the labels of the ``unlabeled set''.  Thus, either authors must manually verify this property, meaning that the learning is not really semi-supervised, or a heavy price may be paid by assuming identities are distinct when in fact they are not. This paper presents a solution to this problem by ....}
%\mc{The introduction does not adequately convey that the paper is geared towards the {\em practice} of face recognition. It is also too matter-of-fact. You should try to convey that exploiting unlabeled data is a big deal and not much is known how to do it in practice, that overlapping identities or pseudolabel noise can significantly impact na\"{i}ve methods, that your experiments are well-designed and improvements are non-trivial. See if you can do a rewrite before I take a pass.}

Deep face recognition has achieved significantly high performance, benefitting from large-scale labeled data, i.e., DeepFace~\cite{deepface} uses 4M labeled faces for training and FaceNet~\cite{schroff2015facenet} is trained on 200M labeled faces. Further improvement in recognition performance requires tremendous annotation efforts in increasing the labeled dataset volume, which is impractical, labor intensive and does not scale well. Therefore, exploring ways and means to exploit unlabeled data has become an attractive alternative. 
% Yet, whether to apply the unlabeled data in an unsupervised way or clustering it with pseudo labels is still under investigation.

%-------------------------------------------------------------------------
\begin{figure}[!!t]
    \centering
    \includegraphics[width=0.85\textwidth]{figures/teaser_fig_v2.pdf}
    \caption{ 
        Given a face recognition model trained on labeled faces, we wish to exploit clustering on unlabeled data for additional training samples to further improve recognition performance. Key challenges include \textit{\textbf{overlapping identities}} between labeled and unlabeled data (circled in red) as well as noisy training labels arising from \textit{\textbf{incorrect cluster assignments}} (a picture of \textit{George Bush Sr.} is erroneously assigned to a cluster of \textit{George W Bush} images).
        } 
    \label{fig:overlap-teaser}
\end{figure}

%Leveraging semi-supervised or unsupervised ways to generate labels on raw faces has thus become an attractive direction~\cite{zhan2018consensus,yang2019learning}.
%
Self-supervised learning utilizes unlabeled data to train deep networks by solving proxy tasks, such as predicting data transformations~\cite{noroozi2016unsupervised,gidaris2018unsupervised,noroozi2018boosting} or clustering~\cite{caron2018deep,caron2019unsupervised}.
%
% Recent self-supervised approaches~\cite{caron2018deep, noroozi2018boosting} apply softmax on top of the K-means clustering to assign category labels, which has shown performance gains for training deep networks.
%
Narrowing the scope to deep face recognition, some preliminary works on generating pseudo-labels from clustering unlabeled faces have been shown to be effective in improving performance~\cite{sohn2018unsupervised,zhan2018consensus,yang2019learning}. 
%
% Inspired by Mask-RCNN~\cite{maskrcnn}, a graph convolutional neural network (GCN) based face clustering method (Face-GCN) is proposed in \cite{yang2019learning} to regress local proposals for the likelihood being within same subject, resolving the scalability issue in GCN for practical applications.
%
However, these methods only consider the cases of newly introduced identities in the unlabeled data, whereas in practice, part of the unlabeled images could share the same identity as existing images in the labeled dataset (Fig.~\ref{fig:overlap-teaser}).
%
% If not merging or removing the overlapped id images from unlabeled data, the clustering will assign those images with a new id, which inevitably introduces significant label noise for the latter recognition training. 
% 
If these overlapping identity images from the unlabeled data are not accounted for, clusters with these images would be considered as new identities, introducing significant label noise into the subsequent re-training of the recognition model.

In this paper, we present recipes for exploiting unlabeled data to improve the performance of face recognition models trained on large-scale labeled datasets, resolving two important practical challenges -- accounting for overlapping identities between labeled and unlabeled data, and attenuating the effect of noisy labels when training on pseudo-labeled data.
%
We begin with Face-GCN \cite{yang2019learning}, a graph convolutional neural network (GCN) based face clustering method, to obtain pseudo-labels on unlabeled faces. To deal with the overlapping identity problem, we observe that the distribution of classification confidence on overlapping and disjoint identities is different -- since our initial face feature is provided by a recognition engine trained on known identities, the confidence score of the overlapping identity images should be higher than those of non-overlapping identity images, as visualized in Fig.~\ref{fig:class-overlap}. 
Based on this observation, we approach the problem as ``out-of-distribution'' detection~\cite{hendrycks2016baseline,liang2017enhancing,lee2018simple}, and propose to parameterize the distribution of confidence scores as a mixture of Weibulls, motivated by extreme value theory. This results in an unsupervised procedure to separate overlapping identity samples from unlabeled data on-the-fly.

After resolving the overlapping id problem, the systematic label noise from the clustering algorithm remains, which is a prime cause for deteriorating performance in face recognition~\cite{wang2018devil}. 
%
Instead of an additional complicated pruning step to discard noisy samples, \eg as done in \cite{yang2019learning}, we deal with the label noise during the re-training of the deep network. Specifically, we introduce a simple clustering uncertainty based weighting on the training loss to reduce the effect of erroneous gradients caused by the noisy labeled data. This effectively smooths the re-training procedure and has shown clear performance gains in our experiments.
%
% \cite{yang2019learning} proposes a second GCN model, termed GCN-S, to prune the proposals and increase the precision or purity of clusters. Training GCN-S requires carefully considering all kinds of outlier situations to prepare training data, which is difficult to replicate and easily results in sensitive predictions. The model complexity is also increased. 
% Instead, we introduce a simple clustering uncertainty based weighting on the training loss to reduce the effect of erroneous gradients caused by the noisy labeled data. This effectively smooths the re-training procedure and has shown clear performance gains in our experiments.

%\mc{This paragraph seems repetitive. Try to summarize main take-aways rather than restating the above technical contributions.}

Our contributions are summarized as follows:
\begin{itemize}
    \item{To our knowledge, we are the first to tackle the practical issue of overlapping identities between labeled and unlabeled faces while clustering, formulated as out-of-distribution detection.}
    
    \item{We propose a simple and scalable uncertainty weighted identification loss for face recognition re-training, designed to compensate for the label noise introduced by the clustering procedure.}
    % which also boosts the recognition performance empirically.}
    
    \item{Extensive experiments on controlled and real-world settings provide useful insights for the practical usage of unlabeled faces and demonstrate that with the proposed clustering and re-training strategies, substantial performance gains over a fully-supervised model are achieved across multiple public face recognition benchmarks, \ie LFW~\cite{huang2008labeled}, YTF~\cite{wolf2011face}, CFP~\cite{sengupta2016frontal} and IJB-A~\cite{kalkaijb}.}
    % and MegaFace~\cite{kemelmacher2016megaface}.}
    
\end{itemize}

%The rest of the paper is organized as follows ... \todo .. 
 


==> suppl_text.tex <==
We include some additional experimental details and discussions here that could not be included in the main paper due to space constraints:
\begin{itemize}
        \item{The overview of approaches on improving face recognition (Sec.~\ref{sec:overview})}
        
        \item{The diversity in datasets (Sec.~\ref{sec:frechet})}
        
        \item{Discussion on the motivation of our choice to model the label noise (Sec.~\ref{sec:uncertain})} 
        
        \item{The effect of the $\gamma$ hyper-parameter on our proposed uncertainty weighted loss  (Sec.~\ref{sec:gamma})} 
        
        \item{Details and baselines for overlapping identity separation (Sec.~\ref{sec:overlap_gaus})}
        
        \item{Visualization of clustering errors and their correspondence to uncertainty scores (Sec.~\ref{sec:cluster_viz})}
        
        \item{Detailed descriptions of the evaluation benchmarks (Sec.~\ref{sec:eval})} 
        
        \item{Implementation details including training settings for the clustering module and the deep face networks (Sec.~\ref{sec:implement})} 
        
\end{itemize}
%\end{abstract}



%%%%%%%%% PREFACE/OVERVIEW
\section{Overview}
\label{sec:overview}
The main submission empirically illustrated the use of unlabeled faces to improve fully-supervised face recognition systems. From the literature, one major direction to boost performance is via \textit{supervised} training, \ie,  leverage various network structures such as VGG Face~\cite{simonyan14very}, ResNet~\cite{he2016deep} and SE-Net~\cite{hu2018squeeze}, or investigating effective objective functions, \ie, triplet loss~\cite{schroff2015facenet}, Cosine Loss~\cite{wang2018cosface}, by constraining the feature lying on a hypersphere~\cite{liu2017sphereface}, or further combine the two~\cite{deng2018arcface}.


Our paper advocates another direction: leverage larger amounts of unlabeled training data in a \textit{semi-supervised} manner. These two axes lead to \textit{orthogonal} developments -- more data is likely to improve the next generation of better face architectures and losses. Moreover, tasks such as automatic adaptation of a model to a new scene or condition will benefit from being able to learn from unlabeled faces. There are several use cases for such adaptation: \eg, a particular ethnicity may not have a large labeled dataset but have many unlabeled faces available. In general, deployed models would be able to leverage a continuous stream of unlabeled data to adapt to specific operational conditions.

% take home msg of main paper here --
We briefly re-iterate our main conclusions here -- the experiments show that it is indeed possible to further improve the recognition performance of fully-supervised models by exploiting clustering to obtain pseudo-labeled additional data. To see significant improvements, we require comparable volumes of labeled and pseudo-labeled data, as well as accounting for label noise and overlapped identities between labeled and unlabeled sets.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{On quantifying the diversity in data}
\label{sec:frechet}

In the large-scale uncontrolled setting experiments presented in the main paper, we observe that samples from a different dataset provides greater benefits w.r.t. performance than more samples drawn from the same distribution as the original labeled training dataset. Intuitively this makes sense -- different datasets would bring in more information that the original network has not seen earlier during training. We quantify this notion of distance or diversity among datasets using a simple Fr\'echet distance~\cite{dowson1982frechet,heusel2017gans}, visualized in  Fig.~\ref{fig:frechet}. The different datasets are arranged along the x-axis based on distance from labeled MS-Celeb.

% \begin{wrapfigure}{r}{0.4\textwidth}
\begin{figure}[!t]
    \centering
    %  \vspace{-8mm}
    \includegraphics[width=0.6\textwidth]{figures/frechet_distance.pdf}
    % \vspace{-8mm}
    \caption{\small{Fr\'echet distance~\cite{dowson1982frechet,heusel2017gans} between MS-1M and the other datasets used as sources of unlabeled data, indicating the domain gap between MS-1M and the unlabeled data.
    %These datasets cover different parts of the feature space than MS-1M, and thus along with increasing the \textit{amount} of training data, they also introduce \textit{diverse} samples.
    }}
    \label{fig:frechet}
    % \vspace{-16mm}
\end{figure}
% \end{wrapfigure}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Motivation of Modeling the Label Noise}
\label{sec:uncertain}

% \noindent \textbf{Choice of linear classifier.} 
Here, we begin by discussing some related work regarding our choice of modeling the noisy labels that may motivate our choice of using a \textit{linear} classifier on top of face descriptor features to decide which cluster assignments are noisy. We note that the label noise from clustering is well-structured, very much unlike the uniform noise (\ie all categories are equally likely to have their correct label flipped) well-studied in the literature on neural network generalization~\cite{zhang2016understanding,arpit2017closer,Forgetting}. 
%
Zhang~\etal~\cite{zhang2016understanding} show that deep neural networks are able to perfectly memorize random labels assigned to the training samples. This would indicate that a network of sufficient expressivity would be able to memorize the incorrect labels in our pseudo-labeled dataset, leading to sub-optimal performance upon re-training with the extra data. Arpit~\etal~\cite{arpit2017closer} however observe that despite the ability to memorize random patterns, deep neural networks tend to learn easy or correctly-labeled patterns first, and then start fitting to the incorrectly labeled examples in subsequent training epochs. \cite{ICML2019_UnsupervisedLabelNoise} report that the training loss of a network on noisy labeled samples is higher than correctly labeled training samples, and this difference can be used to separate out the noisy labels. 

We observe in our initial experiments that at least on our face datasets, the highly-structured labeled noise from clustering assignments behaves differently -- even shallower neural networks were learning to fit to both incorrectly and correctly labeled samples at almost concurrent rates, and thus there was no clear separation by looking at the empirical distribution of the training loss. 
%
\textit{Mixup}~\cite{zhang2017mixup} shows that encouraging deep neural networks to behaving linearly in between samples improves generalization and tolerance to noise.
In fact, \cite{ICML2019_UnsupervisedLabelNoise} report \textit{mixup} regularization to be useful in their label noise robustness experiments. 

%-------------------------------------------------------------
\begin{table}[t]
\renewcommand{\tabcolsep}{5pt}
\centering
\small 
\caption{Effect of tuning hyper-parameter $\gamma$ on the uncertainty weighted loss.
}
\label{tab:gamma_ms1m}
\begin{tabular}{@{\hskip 2mm}l@{\hskip 2mm}c@{\hskip 2mm}c@{\hskip 2mm}c@{\hskip 2mm}c@{\hskip 2mm}c}
\toprule
\textbf{Model}     & \textbf{LFW}  & \textbf{CFP-fp} & \textbf{IJBA-idt.}    & \textbf{IJBA-vrf.}  \\
 & & & Rank-1, 5 & FAR@1e-3,-4 \\
\midrule
Baseline GT-1   & 99.20 & 92.37 & 92.66, 96.42  & 80.23, 69.64  \\
+ GCN           & 99.48 & {95.51} & 94.11, 96.55 & 87.60, 77.67  \\
\midrule
+ GCN $\gamma = \frac{1}{3}$  & {99.60}  & {94.66}    & 94.73, 96.93     &  87.93, 81.16  \\
+ GCN $\gamma = \frac{1}{2}$  & {99.45}  & {92.86}    & 93.47, 96.44     &  84.13, 75.26 \\
+ GCN $\gamma = 1$            & {99.50} & {94.71}     & 94.76, 97.10     &  87.97, 79.43  \\
+ GCN $\gamma = 2$            &  99.48  & {94.71}     & 95.05, 97.26     &  88.43, 79.87  \\
+ GCN $\gamma = 3$            &  99.55  &  94.47      & 94.88, 97.24     &  88.12, 78.74  \\
\midrule
+ GT-2 (bound)    & 99.58 & 95.56 & 95.24, 97.24 & 89.45, 81.02  \\
\bottomrule
\end{tabular}
\end{table}

Our intuition for using linear separability to estimate label noise is as follows -- assuming that effective features have been learned by the baseline model on a large labeled dataset, we trust \textit{only} those cluster assignments that can be fitted by a simple linear classifier on top of these discriminative features. While this does reduce the opportunity of the deep network to learn from some challenging examples (\ie complicated clusters which are not modeled by a simple linear model would have a high loss that may benefit the network), it also reduces the chance of the high losses from incorrectly-clustered samples from destabilizing the network training. 
% Placing our approach within the larger context of generalization, overfitting and classical notions such as cluster-assumption in semi-supervised learning~\cite{chapelle2009semi} is an interesting avenue for future work.

% ------------------------------------------------------------
\section{Effect of Hyper-parameter $\gamma$}
\label{sec:gamma}
%
Setting various values of $\gamma$ in the weighted loss can change the steepness of the weighting curve following a power law: 
$$\mathcal{L}^{p}(\mathbf{x}_i) = (1-p^-(\mathbf{x}_i))^{\gamma}\mathcal{L}(\mathbf{x}_i)$$

The behaviour is somewhat like the ``focusing parameter'' in methods like the focal-loss~\cite{lin2017focal}. However, despite some similarities, the motivation and the implementations are starkly different -- focal loss seeks to emphasize high-loss samples in a training batch, as a means of hard-example mining; we seek to discount the effect of samples which we suspect are incorrectly pseudo-labeled. Moreover, the focal loss uses the deep network's softmax output as the posteriors, while we have a separate parametric model to estimate the probability of an incorrect label.
We show the re-training performance at different values of $\gamma$ in the uncertainty-weighted loss in Table~\ref{tab:gamma_ms1m}. The parametric Weibull model on the classification-margin appears to be a good estimate of this uncertainty, and changing the shape of the curve gives limited benefits. The focusing parameter is observed to have limited effect in practice -- the improvements are not consistent across datasets, and therefore we simply use $\gamma = 1$ in all further experiments. We note that other choices than Weibull, \eg Laplace or beta~\cite{ICML2019_UnsupervisedLabelNoise}, may be used to parameterize this distribution -- our choice was based on the observed skewness of the empirical distribution, which precluded the more common Gaussian.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Overlapping Identity Separation}
\label{sec:overlap_gaus}

%  \arc{why Gaussian does as well -- show that data fit is worse, but thresholds are still good enough} -- \todo --

We show the results of modeling the disjoint/overlapping identity separation as an out-of-distribution problem in Table~\ref{tab:disjoint_overlap}.
%
These results were presented in a much condensed form in the main paper.
%
A simple Otsu's threshold provides acceptably low error rates, i.e., $6.2\%$ false positive rate and $0.69\%$ false negative rate. This shows that our choice of the max-logit score as the feature for OOD is an effective approach.

% ------------------------------------------------------------
\begin{table}[t]
\renewcommand{\tabcolsep}{5pt}
\centering
\small 
\caption{\textbf{Separating overlapped identities.} Results on detecting samples in the unlabeled data whose identity overlaps with classes in the labeled training set.
}
\label{tab:disjoint_overlap}
\begin{tabular}{@{\extracolsep{4pt}}lccc}
\toprule
 \textbf{Method}    & \textbf{False Positives}  & \textbf{False Negatives} & \textbf{SSE} \\
\midrule 
  Naive Otsu        & 6.2\%     & 0.69\%    & - \\
  Gaussian-95\%     & 2.01\%    &   0.51\%  & 0.245 \\
  Weibull-95\%      & 2.33\%    & 0.50\%    & 0.228 \\
\bottomrule
\end{tabular}
\end{table}

Fig.~\ref{fig:overlap_gaussian} shows the Weibull and a baseline Gaussian model fit to the empirical distributions of max-logit scores. We quantify the error in fitting the actual data by the sum-of-squared-errors (SSE) between empirical and theoretical PDFs, shown in the last column of Table~\ref{tab:disjoint_overlap}. The Gaussian model has a slighly higher SSE, indicating a worse fit overall. This justifies the decision to fit the maxima using the Weibull family.

Using $95\%$ confidence intervals from Weibulls, we achieve much lower error rates than the simple Otsu's threshold: ${2.3\%}$ FPR and ${0.50\%}$ FNR. 
Using Gaussians to threshold the max-logits gives almost equivalent results for overlap separation (slightly better in FP and worse in FN), although the Weibulls fit the skewed distributions better.


% --------------
\begin{figure}[t]
    \centering
      \includegraphics[width=0.8\textwidth]{figures/weibull_normal_fit.pdf}
    \caption{Empirical distribution of the max-logit score for overlapping and disjoint identities between labeled and unlabeled sets (shown on controlled splits of MS-1M dataset). The two-component Weibull and Gaussian models are shown in solid lines.}
    \label{fig:overlap_gaussian}
\end{figure}


% \begin{wrapfigure}{r}{0.5\textwidth}
%     \centering
%     % \vspace{-2mm}
%     % \vspace{-0.68cm}
%     \includegraphics[width=0.5\textwidth]{figures/Max-Logit_min-overlap-thresh.pdf}
%     % \vspace{-0.8cm}
%     \caption{ \small{
%     % \textbf{Distribution of max-logits.}
%     Extreme value theory (EVT) provides a principled way of setting thresholds on the max-logits $\boldsymbol{z}_i$ for $\mathbf{x}_i \in \mathcal{X^U}$ to separate \textit{disjoint} and \textit{overlapping} identities ({\color{red}{red}} and {\color{blue}blue} vertical lines). 
%     % An initial threshold is determined by Otsu's method (black vertical line). The true empirical distributions (\textit{overlap-GT} and \textit{disjoint-GT}) are fairly close to the estimated Weibull models (\textit{overlap-Wb} and \textit{disjoint-Wb}). This plot uses splits from the MS-Celeb-1M dataset~\cite{guo2016msceleb}.
%       } } 
%     \label{fig:class-overlap}
%     % \vspace{-1cm}
% \end{wrapfigure}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Visualization of Clustering Errors} 
\label{sec:cluster_viz}
% \arc{samples that are estimated to be incorrectly clustered ... under a unified noise model for both split-identity and outlier samples....} -- \todo --

As discussed in the main paper, our goal is to obtain a model of the noise that can capture the structured label noise resulting from clustering. Re-iterating our steps: \textbf{(1)} train a linear classifier on cluster assignments; \textbf{(2)} define metrics of classification uncertainty such as entropy, classification-margin etc.; \textbf{(3)} to validate the hypothesis, check how well this uncertainty metric corresponds to clustering errors.  


% --------------
\begin{figure}[t]
    \centering
    \begin{tabular}{cc}
      \vspace{-0.1cm}
      \includegraphics[width=0.45\textwidth,trim=0 0 0 1cm, clip]{figures/noisy-label/cluster_noise.pdf} & 
      \includegraphics[width=0.45\textwidth]{figures/noisy-label/pr-curve_log-reg.pdf} \\
      (a) & (b) \\
      \includegraphics[width=0.45\textwidth]{figures/noisy-label/weibull-loss-hist_ms1m-gcn-split-2_err.pdf} &
      \includegraphics[width=0.45\textwidth]{figures/noisy-label/soft-score_ms1m-gcn-split-2_err.pdf} \\
      (c) & (d) \\
    \end{tabular}
    \caption{ \textbf{Clustering uncertainty.}
    \textbf{(a)} Examples of incorrect pseudo-labels -- an image of \textit{George Bush Sr.} is included in a cluster of \textit{George W Bush} images (outlier circled in {\color{blue}blue}); some \textit{George W Bush} images are spread across multiple clusters (``split ID'' circled in {\color{red}red}).
    \textbf{(b)} Precision-recall curves showing Average Precision (AP) of predicting if a cluster assignment is correct using class-margin, max-logit and entropy. 
    \textbf{(c)} Distribution of class-margin with a Weibull fit to the left mode (orange curve).
    \textbf{(d)} An importance weight is assigned to each pseudo-labeled sample based on its likelihood under the Weibull. 
    }
    \label{fig:cluster-err}
\end{figure}




% ------------------------------------------------------------
\begin{figure*}[!!tp]
    \centering
     \qquad Inliers \qquad \qquad  \qquad  \qquad  \qquad  \qquad Outliers \\
    \includegraphics[width=0.65\textwidth]{figures/images/cluster-noise-outliers/cluster_noise_faces-outliers_1.pdf} \\
    \includegraphics[width=0.65\textwidth]{figures/images/cluster-noise-outliers/cluster_noise_faces-outliers_2.pdf} \\
    \includegraphics[width=0.65\textwidth]{figures/images/cluster-noise-outliers/cluster_noise_faces-outliers_3.pdf} \\
    \includegraphics[width=0.65\textwidth]{figures/images/cluster-noise-outliers/cluster_noise_faces-outliers_4.pdf} \\
    \includegraphics[width=0.65\textwidth]{figures/images/cluster-noise-outliers/cluster_noise_faces-outliers_5.pdf} \\
    \caption{ \textbf{Cluster outliers.} The \textbf{\textit{left column}} shows inlier samples from 5 clusters. The \textbf{\textit{right column}} shows faces of \textit{different identity} being assigned to the \textit{same cluster} as on the left (outlier samples).  
    The numbers below show the mean and standard deviation of the likelihood of being a noisy label ($p^-$). Note that the outlier samples on the right on average have significantly higher likelihood under this noise model. 
    Having a distinctive common attribute like eye-glasses (\textit{row 2}), facial hair (\textit{row 3}) or prominent eyebrows (\textit{last row}) can confound the clustering, even though the identities are different.
     }
    \label{fig:cluster-outlier}
\end{figure*}


% ------------------------------------------------------------
\begin{figure*}[tp]
    \centering
    \qquad True ID \qquad \qquad  \qquad  \qquad  \qquad  \qquad Split-ID \\
    \includegraphics[width=0.65\textwidth]{figures/images/cluster-noise-split-id/cluster_noise_faces-split-ID_1.pdf} \\
    \includegraphics[width=0.65\textwidth]{figures/images/cluster-noise-split-id/cluster_noise_faces-split-ID_2.pdf} \\
    \includegraphics[width=0.65\textwidth]{figures/images/cluster-noise-split-id/cluster_noise_faces-split-ID_3.pdf} \\
    \includegraphics[width=0.65\textwidth]{figures/images/cluster-noise-split-id/cluster_noise_faces-split-ID_4.pdf} \\
    \includegraphics[width=0.65\textwidth]{figures/images/cluster-noise-split-id/cluster_noise_faces-split-ID_5.pdf}
    \caption{ \textbf{Split-identity clustering.} The \textbf{\textit{left column}} shows samples from 5 clusters. The \textbf{\textit{right column}} shows faces that share the \textit{same identity} as on the left, but have been assigned to \textit{different clusters}. The numbers below show the mean and standard deviation of the likelihood of being a noisy label ($p^-$). Note that the ``split identity'' samples on the right, that have been separated from the ``true cluster'' of that identity, have higher values under this noise model.
    E.g. \textit{top row:} all images belong to the same person (actor Max von Sydow), but due to factors such as age and facial hair, all images are not assigned the same cluster.
     }
    \label{fig:cluster-split-id}
\end{figure*}

To this end, we attempt to quantify the typical errors that occur in cluster assignments (Fig.~\ref{fig:cluster-err})~\footnote{We repeat this figure here from the main paper for ease of exposition in the writing.}, based off the standard metrics of precision and recall:

\begin{itemize}
        \item{\textbf{\textit{Outliers:}} Using ground-truth labels, we first find the modal or most frequent  identity in a cluster. Samples corresponding to this identity are \textit{inliers}. The others are \textit{outliers}. This type of error affects the precision of the clustering algorithm. Some illustrative examples from the MS-1M splits are shown in Fig.~\ref{fig:cluster-outlier}, where each row depicts a cluster. The clustering algorithm confuses matching attributes like facial hair, sunglasses, heavy eyebrows etc. for identity, and ends up putting different people into the same cluster.}
        
        \item{\textbf{\textit{Split-identity:}} This type of error occurs when samples from the \textit{same} identity as split across \textit{different} clusters, which impacts the recall metric of a clustering algorithm. For a ground-truth identity, we find all clusters that contain samples belonging to this identity. A perfect clustering would assign all samples of a person to a \textit{single} cluster, but this is generally not the case -- samples of a person can be scattered or split over several clusters~\footnote{Note that Face-GCN typically has very high precision, but comparatively lower recall, which is why this type of error is more common in our experiments.}. We find the cluster with the highest number of samples for a particular identity, regarding it as the ``true cluster'', and the other clusters as having incorrectly split the identity (this is a rough heuristic that we empirically found to be feasible). Some examples of this scenario are shown in Fig.~\ref{fig:cluster-split-id}. E.g. the first row shows various images of the Swedish actor \href{https://www.imdb.com/name/nm0001884/?ref_=nmbio_bio_nm}{Max von Sydow}. Most of his middle-aged and older images form the largest or ``true'' cluster, shown on the left. Several images that exhibit other attributes like facial hair or a much younger age end up forming separate clusters, as shown on the right.} 
\end{itemize}
    
    
    
    
% --------------------------------------------------------------
As detailed in the main paper, we use precision-recall curves to analyse the correspondence of our uncertainty metrics with clustering errors, finding the highest Average Precision (AP) with \textit{\textbf{classification-margin}} (95.16\%), with \textit{max-logits} and softmax \textit{entropy} getting APs of 94.80\% and 88.29\%, respectively. The empirical distribution of classification-margin scores on a noisy dataset was observed to be bi-modal -- incorrect clusterings had a small classification-margin since they were difficult for the logistic regression classifier to learn correctly. In Fig.~\ref{fig:cluster-err}(b), a Weibull distribution fit to the lower mode gives our noise model $p^{-}(\mathbf{x}_i)$, \ie the likelihood that a sample $\mathbf{x}_i$ has been clustered incorrectly. Figures~\ref{fig:cluster-outlier} and \ref{fig:cluster-split-id} also show the average values of $p^{-}(\mathbf{x}_i)$ for the samples -- inliers and true-clusters are typically given a lower likelihood under this model, \ie we are \textit{less} uncertain about their cluster assignment. 





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Evaluation Benchmarks}
\label{sec:eval}
The main paper presents results on the following benchmarks, which we describe in more details here: 

\begin{itemize}
    \item{\textit{\textbf{Labeled Faces in the Wild (LFW)}}~\cite{huang2008labeled,learned2016labeled}: consists of 13,233 images and 5749 people, reporting verification accuracy across 10 folds of 300 matching and 300 non-matching face pairs.} 
    
    \item{\textit{\textbf{Celebrity Frontal to Profile (CFP)}}~\cite{sengupta2016frontal}: consists of 500 people, each with 10 frontal and 4 profile images. There are two verification protocols -- frontal to frontal (\textit{ff}) and frontal to profile (\textit{fp}) images. Each protocol consists of 10 folds with 350 same-identity and mismatched-identity pairs.}
    
    % \item{ \textit{\textbf{YouTube Faces (YTF)}}~\cite{wolf2011face}: consists of 3,425 videos of 1,595 people. 2500 same-identity pairs and 2500 mismatched-identity pairs are divided into 10 splits.}
    
    \item{\textit{\textbf{IJB-A}}~\cite{klare2015pushing}:  part of the challenging IARPA Janus benchmark, it has 500 subjects with 5,397  images and 2,042 videos. Identification performance is reported as retrieval rate at ranks 1 and 5, using 10 splits each with 112 gallery templates and 1763 probe templates (\ie 1,187  genuine queries and 576 impostor queries whose identities are not in the gallery). Verification performance is reported as True Accept Rate (TAR) at False Accept Rates (FAR) ranging from 1e-1 to 1e-4, evaluated on 10 splits with 11,748 pairs of templates (1,756 positive and 9,992 negative pairs); we report performance at the two most strict settings: FAR@1e-3,1e-4 respectively.} 
\end{itemize}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Implementation Details}
\label{sec:implement}
\noindent
\textbf{Face recognition training.} 
The CosFace model~\cite{wang2018cosface} is used as our face recognition engine, which is one of the top performance methods on standard face recognition benchmarks. A 118-layer ResNet is used as the backbone network. 
The baseline model on labeled data is trained for 30 epochs using SGD with momentum $0.95$, with a batch size of 512 across 8 GPUs in parallel, starting from a learning rate of 0.1, with the learning rate dropping by a factor of $1/10$ at the $16^{th}$ and $23^{rd}$ epochs.  When used as a feature extractor, this model yields vectors of 512 dimensions. When training with pseudo-labeled data, we re-train the entire model from scratch on the union of the labeled and pseudo-labeled data, with the same training settings. 

\noindent
\textbf{Clustering model training.} The Face-GCN implementation uses the publicly available code~\footnote{\url{https://github.com/yl-1993/learn-to-cluster}} of GCN-D from \cite{yang2019learning}. An initial k-nearest neighbor graph is formed over the unlabeled samples with $k=80$, using the \href{https://github.com/facebookresearch/faiss/wiki}{FAISS} library for efficient similarity computation over large sample sizes. Cluster proposals are generated from this by setting various thresholds -- we find optimal settings on a held-out set of MS-Celeb-1M and continue to use these consistently on all the other datasets. The \texttt{GCN-D} model from Face-GCN is trained to predict the precision and/or recall for each cluster proposal. We use a simple 3-layer architecture, with feature sizes: $512 \rightarrow 256 \rightarrow 64$, following by a global max-pooling. Following \cite{yang2019learning}, the model is trained with a regression loss.

\noindent
\textbf{Re-training on pseudo-labels.} Following the final clustering output from Face-GCN, we discard clusters with fewer than 10 samples as a simple heuristic. The remaining cluster assignments on the remaining samples are treated as category labels and merged with the labeled training set. To control for different optimization settings and validation sets, we simply re-train the face recognition model, from scratch, with the same number of epochs and learning rate schedule as the baseline model trained on labeled data -- therefore, the only change between the baseline model and the re-trained model is the extra pseudo-labeled training data.
